On the Generalization Ability of Unsupervised Pretraining

Recent advances in unsupervised learning have shown that unsupervised pre-training, followed by fine-tuning, can improve model generalization. However, a rigorous understanding of how the representation function learned on an unlabeled dataset affects the generalization of the fine-tuned model is lacking. Existing theoretical research does not adequately account for the heterogeneity of the distribution and tasks in pre-training and fine-tuning stage. To bridge this gap, this paper introduces a novel theoretical framework that illuminates the critical factor influencing the transferability of knowledge acquired during unsupervised pre-training to the subsequent fine-tuning phase, ultimately affecting the generalization capabilities of the fine-tuned model on downstream tasks. We apply our theoretical framework to analyze generalization bound of two distinct scenarios: Context Encoder pre-training with deep neural networks and Masked Autoencoder pre-training with deep transformers, followed by fine-tuning on a binary classification task. Finally, inspired by our findings, we propose a novel regularization method during pre-training to further enhances the generalization of fine-tuned model. Overall, our results contribute to a better understanding of unsupervised pre-training and fine-tuning paradigm, and can shed light on the design of more effective pre-training algorithms.

==> acknowledge.tex <==
\section*{Acknowledgement}
We would like to thank Mohammad Mahdi Kamani for his help on conducting the experiments. We would also like to thank an anonymous reviewer from ICML 2021 for pointing out an issue of the assumption on $\phi$ in the previous version of this manuscript.

==> backup_of_proof.tex <==
\paragraph{Upper bounding $\Delta^{ft}_{\cU}(\hat{h}, h^*_{\cU})$}
We examine $\Delta^{ft}_{\cU}(\hat{h}, h^*_{\cU})$ first. Similar to DAE proof, We define the optimal head for classification task on distribution $\cU_{\cX}$ under representation $h^*_{\cU}$ as $\tilde\btheta^* = \arg\min_{\norm{\tilde\btheta}\leq  R} \E_{\tilde\mZ  \sim \cU_{\cX}}[\phi(\tilde{\btheta}^\top   (\be_1^\top   {h}^*_{\cU} (\tilde\mZ )  )   )]$.
\begin{align*}
    &\Delta^{ft}_{\cU}(\hat{h}, h^*_{\cU}) =  \min_{\norm{\btheta}\leq R} \E_{(\tilde\mZ ,\mZ)\sim \cU }[\phi(\btheta^\top (\be_1^\top \hat{h}(\tilde\mZ) )^\top  )]-  \E_{(\tilde\mZ ,\mZ)\sim \cU }[\phi({\tilde \btheta }^{\star \top}     (\be_1^\top{h}^*_{\cU} (\tilde\mZ)  )^\top   )]\\
    &\leq  \min_{\norm{\btheta}\leq R} G_\phi \E_{(\tilde\mZ ,\mZ)\sim \cU }| (\btheta^\top  (\be_1^\top \hat{h}(\tilde\mZ) )^\top   ) -    ({\tilde \btheta }^{\star \top}    (\be_1^\top h^*_{\cU}(\tilde\mZ) )^\top    )|\\
    &\leq  \min_{\norm{\btheta}\leq R} G_\phi \sqrt{\E_{(\tilde\mZ ,\mZ)\sim \cU }\pare{ \btheta^\top (\be_1^\top \hat{h}(\tilde\mZ) )^\top   -    {\tilde \btheta }^{\star \top}    (\be_1^\top {h}^*_{\cU}(\tilde\mZ) )^\top     }^2}\\
    &=  \min_{\norm{\btheta}\leq R} \\
    &\quad  G_\phi\sqrt{   \btheta^\top \E\left[ (\be_1^\top \hat{h}(\tilde\mZ) )^\top (\be_1^\top \hat{h}(\tilde\mZ) )\right] \btheta   - 2 \btheta^\top  \E\left[(\be_1^\top \hat{h}(\tilde\mZ) )^\top (\be_1^\top  {h}^*_{\cU}(\tilde\mZ) ) \right]\tilde{\btheta}^\top       +  {\tilde \btheta }^{\star \top} \E\left[(\be_1^\top  {h}^*_{\cU}(\tilde\mZ) )^\top(\be_1^\top \hat{h}^*_{\cU}(\tilde\mZ) ) \right] \tilde{\btheta}  }
\end{align*}
Since $\sqrt{f(x)}$ and $f(x)$ attain the minimum at the same point, we examine the minimum of above statement over $ \btheta$ without square root. Under unconstrained setting, the minimum of above statement is $  {\tilde \btheta }^{\star \top} \Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)}   \tilde\btheta^*$ when $ \btheta^* = \pare{\E\left[ (\be_1^\top \hat{h}(\mX) )^\top (\be_1^\top \hat{h}(\mX) )\right]}^{\dagger}\E\left[(\be_1^\top \hat{h}(\mX) )^\top (\be_1^\top  {h}^*_{\cU}(\mX) )\right] \tilde\btheta^*$.
Hence we have 
\begin{align*}
    \Delta^{ft}_{\cU}(\hat{h}, h^*_{\cU})  &\leq    \sqrt{{\tilde \btheta }^{\star \top} \Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)} \tilde\btheta^*  } = \sqrt{\trace(\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)}\tilde\btheta^*{\tilde \btheta }^{\star \top} )}\\
    &\leq  \sqrt{ d\sigma_{\max}(\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)}) \sigma_{\max}(\tilde\btheta^*{\tilde \btheta }^{\star \top}) },
\end{align*}
where 
\begin{align*}
    &\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)} \\
    &=  \E\left[(\be_1^\top  {h}^*_{\cU}(\mX) )^\top(\be_1^\top  {h}^*_{\cU}(\mX) )\right] -\E\left[(\be_1^\top \hat{h}(\mX) )^\top (\be_1^\top  {h}^*_{\cU}(\mX) ) \right]\pare{\E\left[(\be_1^\top \hat{h}(\mX) )^\top (\be_1^\top \hat{h}(\mX) )\right] }^{\dagger}\E\left[(\be_1^\top \hat{h}(\mX) )^\top (\be_1^\top  {h}^*_{\cU}(\mX) )  \right] . 
\end{align*} 
 

At last, by choosing a properly large $R$, we can guarantee the optimum can be attained.

\paragraph{Lower bounding $\Delta^{pt}_{\cU}(\hat{h}, h^*_{\cU})$}

Notice that in masked pre-training, the output of encoder is length $K'$ sequence, i.e., $h(\widetilde\mZ)\in \R^{K'\times d}$, where $K'$ is the number of unmasked patches. Hence we use 
${h}_{\texttt{Aug}} (\widetilde\mZ)\in \R^{K\times d}$ to denote the augmented version of the encoded patches in ${h}  (\widetilde\mZ) \in \R^{(K')\times d}$ where the missing patches are filled by zero vectors.

We define $ h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw$ to be the padded version of ${h}_{\textrm{Aug}} (\widetilde\mX) $, where the masked (zero) patches in ${h}_{\texttt{Aug}} (\widetilde\mX)$ is padded by vector $\bw_{\texttt{Pad}}\in\R^d$.

\begin{align*}
    & \Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU})\\
   &= \min_{\mW_Q^D,\mW_K^D,\mW_V^D  } \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{  \text{softmax}\pare{\frac{ (\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}})\mW_Q^D ((\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}})\mW_K^D)^\top}{\sqrt{d_K}}} (\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}}) \mW_{V}^D  -\mX }_{\mathrm{F}}^2 \\
   &\quad - \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{ \text{softmax}\pare{\frac{  (h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}){\mW_Q^D}^* ((h^*_{\texttt{Aug}} (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}){\mW_K^D}^*)^\top}{\sqrt{d_K}}} (h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}) {\mW_{V}^D }^*  -\mX }_{\mathrm{F}}^2\\
   &\geq \min_{\mS\in\cS, \norm{\mW^D_V}\leq W(L+1)} \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{ \mS (\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}})\mW^D_V -\mX }_{\mathrm{F}}^2  - \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{ \mS^*_{\widetilde \mZ}(h^*_{\texttt{Aug}}  (\widetilde \mZ) \bigoplus \bw_{\texttt{Pad}})  {\mW_{V}^D }^* -\mX }_{\mathrm{F}}^2,
\end{align*}
 where
$\cS$ is the set of all real valued matrices, whose row are from $K$ dimensional simplex:
\begin{align*}
    \cS := \{\mS\in\R^{K\times K}: \bs_i \in \cC^K, \forall i \in [K] \},
\end{align*}
and for notational convenience, we defined:
\begin{align*}
    \mS^*_{\widetilde \mZ} := \text{softmax}\pare{\frac{  (h^*_{\texttt{Aug}}  (\widetilde \mZ) \bigoplus \bw_{\texttt{Pad}}){\mW_Q^D}^* ((h^*_{\texttt{Aug}} (\widetilde \mZ) \bigoplus \bw_{\texttt{Pad}}){\mW_K^D}^*)^\top}{\sqrt{d_K}}} 
\end{align*}


Due to our Assumption~\ref{assumption: realizable}, the optimal encoder-decoder in the hypothesis class which can perfectly recover masked data, with unbiased noise, we have
\begin{align*}
    \E_{(\tilde\mZ ,\mZ)\sim \cU } \left[  \mS^*_{\widetilde\mZ} (h^*_{\texttt{Aug}}  (\tilde\mZ) \bigoplus \bw_{\texttt{Pad}}) {\mW_{V}^D }^* -\mZ  \right] = 0.
\end{align*}
 

Hence
\begin{align*}
    \Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU}) & \geq 
      \min_{\mS\in\cS, \mW^D_V} \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{ \mS\cdot(\hat h_{\texttt{Aug}}(\tilde\mZ)\bigoplus \bw_{\texttt{Pad}}) \mW^D_V - \mS^*_{\tilde\mZ}(h^*_{\texttt{Aug}}  (\tilde\mZ) \bigoplus \bw_{\texttt{Pad}})  {\mW_{V}^D }^*  }^2_{\mathrm{F}}\\
     & \geq \sum_{i\in[K]} \min_{\bs_i \in \cC^K, \mW^D_V } \E_{(\tilde\mZ ,\mZ)\sim \cU }\norm{ \bs_i^\top(\hat h_{\texttt{Aug}}(\tilde\mZ)\bigoplus \bw_{\texttt{Pad}}) \mW - {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}})  {\mW_{V}^D }^*  }^2\\
      & \geq \sum_{i\in[K]} \sum_{j\in [d]} \min_{\bs_i \in \cC^K, \bw_j} \E_{(\tilde\mZ ,\mZ)\sim \cU }\pare{ \bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}}) \bw_j - {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}) \bw_j^*  }^2.
\end{align*}
where we use $\bw_j$ to denote each row of $\mW^D_V$, $\bw_j^*$ to denote each row of $\mW^{D*}_V$ and $\bs_i$ to denote each row of $\mS$, and $\bs_i^*$ to denote each row of $\mS^*$.
Now, let define $\mW_{\texttt{Pad}} \in \R^{K  \times d}$ are the matrix such that its $i$th row equal to $ \bw_{\texttt{Pad}}$, if row $i$ is missing patch in $\hat h_{\texttt{Aug}}(\widetilde \mX)$, otherwise is $\mathbf 0$.
% To further reduce notational complexity, we define $v^*_{ij} = {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}})  \bw_j^*$
We define $$\hat\bs_i^* = \arg\min_{\bs_i \in \cC^K} \min_{\bw_j:\norm{\bw_j}\leq W} \E_{(\tilde\mZ ,\mZ)\sim \cU }\pare{ \bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)\bigoplus \bw_{\texttt{Pad}}) \bw_j - {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}) \bw_j^*}^2 $$.
Then we can further lower bound $\Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU})$:
\begin{align*}
    &\Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU})  \\
      & \geq \sum_{i\in[K]} \sum_{j\in [d]} \min_{\norm{\bw_j}\leq W(L+1) } \E\pare{ \hat\bs_i^{* \top}(\hat h_{\texttt{Aug}}(\widetilde \mZ)+ \mW_{\texttt{Pad}}) \bw_j - {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}) \bw_j^*   }^2\\
      & \geq \frac{1}{2}\sum_{i\in[K]} \sum_{j\in [d]} \min_{ \norm{\bw_j}\leq W(L+1) } \E\pare{ \hat\bs_i^{* \top} \hat h_{\texttt{Aug}}(\widetilde \mZ) \bw_j - {\bs^*_i}^\top h^*_{\texttt{Aug}}  (\widetilde \mZ)  \bw_j^* }^2 \\
      &\quad - \sum_{i\in[K]} \sum_{j\in [d]} \min_{ \norm{\bw_j}\leq W(L+1) } \pare{ \hat\bs_i^{* \top} \mW_{\texttt{Pad}}  \bw_j  -{\bs^*_i}^\top \mW_{\texttt{Pad}}  \bw_j^* }^2\\
      & \geq \frac{1}{2}\sum_{i\in[K]} \sum_{j\in [d]} \min_{ \norm{\bw_j}\leq W(L+1)} \E\pare{\hat\bs_i^{* \top} \hat h_{\texttt{Aug}}(\widetilde \mZ) \bw_j - {\bs^*_i}^\top(h^*_{\texttt{Aug}}  (\widetilde \mX) \bigoplus \bw_{\texttt{Pad}}) \bw_j^*   }^2 - 2Kd \pare{K' \norm{\bw_{\texttt{Pad}} } W(L+1)  }^2\\
      & \geq  \sum_{i\in[K]} \sum_{j\in [d]} \min_{\bs_i \in \cC^K,  {\bw_j} \in \R^d } \\
      &\quad \E\pare{ \bw_j^\top(\hat h_{\texttt{Aug}}( \tilde\mZ) )^\top   \bs_i^{* }\hat\bs_i^{* \top}  \hat h_{\texttt{Aug}}( \tilde \mZ)  \bw_j - 2 \bw^*_j^\top(  h^*_{\texttt{Aug}}( \tilde \mZ) )^\top\hat\bs_i^{* }\hat\bs_i^{* \top} \hat h_{\texttt{Aug}}( \tilde \mZ) \bw_j  + \bw^*_j^\top(  h^*_{\texttt{Aug}}(\tilde \mZ) )^\top \bs_i^{* } \bs_i^{* \top}   h^*_{\texttt{Aug}}( \tilde \mZ) \bw_j^* } \\
      &\quad  -   \frac{2K^3d^2W\cdot W(L+1)}{N}.   
\end{align*}
Similar to DAE proof, we define Schur complement as:
 
\begin{align*}
    &\Lambda\pare{\hat\bs_i^{* \top}\hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs_i^\top h^*_{\texttt{Aug}}(\tilde \mZ)}\\
    &= \E\left[( h^*_{\texttt{Aug}}( \tilde\mZ) )^\top \bs_i^{* } \bs_i^{* \top}  h^*_{\texttt{Aug}}( \tilde \mZ)\right] \\
    &\quad -\E\left[({h}^*_{\texttt{Aug}}(\tilde\mZ))^\top\bs^{*}_i\hat\bs_i^{* \top} (\hat h_{\texttt{Aug}}( \tilde\mZ) ) \right]\pare{\E\left[( h^*_{\texttt{Aug}}( \tilde\mZ) )^\top\bs^*_i \bs^*_i{{h}^*_{\texttt{Aug}}}^\top(\tilde\mZ) \right] }^{\dagger}\E\left[(\hat h_{\texttt{Aug}}( \tilde\mZ) )^\top\bs_i \bs^{*\top}_i{{h}^*_{\texttt{Aug}}}(\tilde\mZ) \right] . 
\end{align*}
 By computing the closed form solution of quadratic form we arrived at:
\begin{align*}
       \Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU})    & \geq       \sum_{i=1}^K\sum_{j=1}^d  \bw_j^{*\top} \Lambda\pare{\hat\bs^{*\top}_i \hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs^{*\top}_i  h^*_{\texttt{Aug}}(\tilde \mZ)} \bw_j^*   \\ 
     & \geq  \sum_{i=1}^K \textrm{tr}\pare{ \Lambda\left(\hat\bs^{*\top}_i \hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs_i^{*\top} h^*_{\texttt{Aug}}(\tilde \mZ)\right)    \sum_{j=1}^d\bw_j^* \bw_j^{*\top}}  \\
     &\geq  \sum_{i=1}^K \sigma_{\max}\pare{\Lambda\pare{\hat\bs^{*\top}_i \hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs_i^{*\top} h^*_{\texttt{Aug}}(\tilde \mZ)} } \sigma_{\min}\pare{ \sum_{j=1}^d\bw_j^*\bw_j^{*\top}}  
\end{align*}
 Recall that 
 \begin{align*}
     \Delta^{ft}_{\cU} (\hat{h}, h^*_{\cU}) \leq \sqrt{d \sigma_{\max}\pare{\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)}} \sigma_{\max}(\tilde\btheta^*{\tilde \btheta }^{\star \top}) }.
 \end{align*}
Hence, we can conlude that
\begin{align*}
   \frac{\Delta^{ft}_{\cU} (\hat{h}, h^*_{\cU}) }{\pare{\Delta^{pt}_{\cU} (\hat{h}, h^*_{\cU})+ \frac{2K^3d^2W^2(L+1)}{N}}^{1/2}    }  \leq O\pare{\frac{ \sqrt{  \sigma_{\max}\pare{\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*_{\cU}(\tilde \mZ)}}  }}{\sqrt{\sum_{i=1}^K \sigma_{\max}\pare{\Lambda\pare{\hat\bs^{*\top}_i \hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs_i^{*\top} h^*_{\texttt{Aug}}(\tilde \mZ)} } } } \sqrt{\frac{d\sigma_{\max}(\tilde\btheta^*{\tilde \btheta }^{\star \top})}{\sigma_{\min}\pare{ \sum_{j=1}^d\bw_j^*\bw_j^{*\top}}}}},
\end{align*}
which indicates that MAE pre-training admits an
$$\pare{\Omega\pare{\frac{ \sqrt{  \sigma_{\max}(\Lambda\pare{\be^{ \top}_1 \hat{h}(\tilde \mZ),\be_1^{ \top} h^*(\tilde \mZ)})  }}{\sqrt{\sum_{i=1}^K \sigma_{\max}\pare{\Lambda\pare{\hat\bs^{*\top}_i \hat{h}_{\texttt{Aug}}(\tilde \mZ),\bs_i^{*\top} h^*_{\texttt{Aug}}(\tilde \mZ)} } } }  },\frac{1}{2}}$$

Bernstein transferrability to binary classification task with bias  $\frac{2K^3d^2W^2(L+1)}{N}$. Notice that the transfer constant $C_{\beta}$ mainly depends on the {\em skewness} of $\bs_i^*$ and $\hat{\bs}_i^*$ w.r.t. $\be_1$. When $\bs_i^*$ and $\hat{\bs}_i^*$ are close to $\be_1$, the $C_{\beta}$ will be small. Otherwise, it will be large. In the main paper Lemma~\ref{lem:MAE transfer} we omit the constant dependency.

% \begin{lemma}
% For any $h\in\cH$, we have:
%    \begin{align*}
%       \E_{\cM} \norm{ h_{\texttt{Aug}} (\widetilde \mX) + \mW  } \leq \norm{ \mW_V}^2  ((K-1)p^2 + pK)\norm{\mX}^2_{\mathrm{F}} + K(1-p)\norm{\bw}^2.
%    \end{align*}
%    \begin{proof}
%    \begin{align*}
%         \E_{\cM} \norm{h_{\texttt{Aug}} (\widetilde \mX) + \mW  }^2  
%         &=\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}}\norm{h^{(i)}_{\texttt{Aug}} (\widetilde \mX)  }^2 + \ind{i\notin \mathcal{E}}\norm{\bw }^2 \\
%    \end{align*} 
%       We can further expand:
%         \begin{align*}
%          \norm{h^{(i)}_{\texttt{Aug}} (\widetilde \mX)  }^2  &= \norm{\text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{   (\bx^{(i)})^\top     \widehat{\mW}_Q   }{  \widetilde \mX {\widehat{\mW}_K}  }}\widetilde \mX  \widehat{\mW}_{V}  }^2 \leq  \norm{\widetilde \mX}^2 \norm{\widehat\mW_V}^2  
%       \end{align*}
%     Plugging it back yields:
%     \begin{align*}
%          \E_{\cM} \norm{h_{\texttt{Aug}} (\widetilde \mX) + \mW  }^2  
%         &\leq \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}}\norm{\widetilde \mX}^2 \norm{ \mW_V}^2 + \ind{i\notin \mathcal{E}}\norm{\bw }^2 \\
%         &=\norm{ \mW_V}^2\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}}\sum_{j=1}^K \ind{j\in \mathcal{E}} \norm{\bx^{(j)}}^2 + \ind{i\notin \mathcal{E}}\norm{\bw }^2 \\
%         & = \norm{ \mW_V}^2 \sum_{j=1}^K ((K-1)p^2 + pK)\norm{\bx^{(j)}}^2 + K(1-p)\norm{\bw}^2\\
%            & = \norm{ \mW_V}^2  ((K-1)p^2 + pK)\norm{\mX}^2_{\mathrm{F}} + K(1-p)\norm{\bw}^2.
%     \end{align*}
      
 
%    \end{proof}
% \end{lemma}

% \begin{lemma}
% For any $h\in\cH$
%    \begin{align*}
%       \E_{\cM} \norm{( {h}_{\texttt{Aug}} (\widetilde \mX) + \mW) - q {h}(\mX)} \leq &2\pare{p(1-q)^2 + p^2 (K-1)(1-q)^2 + pq^2(K-1)(1-p)} \norm{\mX}_{\mathrm{F}}^2\\
%           &+ \frac{2pq^2(1-p)}{\tau^2 d_K} \norm{\mW_K}^2 \norm{\mW_V}^2 \norm{\mX}_{\mathrm{F}}^6  +2 \norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2 p(1-q)^2 \norm{\mX}_{\mathrm{F}}^2  \\
%           &+ 2(1-p) \pare{ K\norm{\bw}^2 - q\sum_{i=1}^K \bw^\top {h}^{(i)}(\mX)  + q^2 \norm{h(\mX)}^2_{\mathrm{F}} }.
%    \end{align*}
%    \begin{proof}
%    \begin{align*}
%         \E_{\cM} \norm{({h}_{\texttt{Aug}} (\widetilde \mX) + \mW) - q{h}(\mX)}^2 &\leq  \E_{\cM} \sum_{i=1}^K\norm{({h}^{(i)}_{\texttt{Aug}} (\widetilde \mX) + \bw) -q{h}^{(i)}(\mX)}^2\\
%         &=\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}}\norm{{h}^{(i)}_{\texttt{Aug}} (\widetilde \mX) - q{h}^{(i)}(\mX)}^2 + \ind{i\notin \mathcal{E}}\norm{\bw - q{h}^{(i)}(\mX)}^2 \\
%    \end{align*}
%       % \begin{align*}
%       %    \norm{\hat{h}^{(i)}_{\texttt{Aug}} (\widetilde \mX) - \hat{h}^{(i)}(\mX)}^2 = \norm{(\widetilde\mS \widetilde \mX\widehat{\mW}_{V})^{(i')}  - (\mS  \mX  \widehat{\mW}_{V})^{(i)} }^2 
%       % \end{align*}
%       % where $\widetilde \mS = \text{softmax}\pare{\frac{      \widetilde \mX    {\widehat{\mW}_Q}  ( \widetilde \mX {\widehat{\mW}_K} )^\top}{\sqrt{d_K}}} $, $ \mS = \text{softmax}\pare{\frac{ \mX    {\widehat{\mW}_Q}  ( \mX {\widehat{\mW}_K} )^\top}{\sqrt{d_K}}} $.
%       We can further expand:
%         \begin{align*}
%         &  \norm{{h}^{(i)}_{\texttt{Aug}} (\widetilde \mX) - q{h}^{(i)}(\mX)}^2 \\
%          &\leq \norm{\text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{   (\bx^{(i)})^\top    {\mW}_Q   }{  \widetilde \mX {{\mW}_K}  }}\widetilde \mX_{\texttt{Aug}}  {\mW}_{V} +\widetilde \mX_{\texttt{Aug}}  - \text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{ (\bx^{(i)} )^\top    {\mW}_Q   }{    q\mX {{\mW}_K}  }}  \mX  {\mW}_{V}- q\mX}^2 \\
%          &\quad \cdot \norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2 \\
%          &\leq 2\underbrace{\norm{\text{Softmax}\pare{\frac{\inprod{   (\bx^{(i)})^\top     {\mW}_Q   }{  \widetilde \mX {{\mW}_K}  }}{\sqrt{d_K}}}\widetilde \mX_{\texttt{Aug}}  {\mW}_{V}    - \text{Softmax}\pare{\frac{\inprod{ (\bx^{(i)} )^\top    {\mW}_Q   }{    \mX {{\mW}_K}  }}{\sqrt{d_K}}}  q\mX  {\mW}_{V}}^2}_{T_1}\norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2\\
%          &+2\norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2 \norm{\ind{i\in\mathcal{E}}\bx^{(i)}- q\bx^{(i)}}^2 \\ 
%          % &\leq   \norm{ \sum_{j\in \mathcal{E}} 
%          %   \frac{\exp\pare{(\bx^{(i)})^\top     \widehat{\mW}_Q\widehat{\mW}_Q^\top \bx^{(j)} /\tau }}{ \sum_{j'\in \mathcal{E}} \exp\pare{(\bx^{(i)})^\top     \widehat{\mW}_Q\widehat{\mW}_Q^\top \bx^{(j')} /\tau }  }  (\bx^{(j)}  )^\top\widehat{\mW}_{V} - \sum_{j=1}^K 
%          %   \frac{\exp\pare{(\bx^{(i)})^\top     \widehat{\mW}_Q\widehat{\mW}_Q^\top \bx^{(j)} /\tau }}{ \sum_{j'=1}^K \exp\pare{(\bx^{(i)})^\top     \widehat{\mW}_Q\widehat{\mW}_Q^\top \bx^{(j')} /\tau }  }  (\bx^{(j)}  )^\top\widehat{\mW}_{V}}^2 \\
%       \end{align*}
%     We define $\widetilde{\mX}_{\texttt{Aug}} \in \R^{K\times d}$ as the augmented version of $\tilde\mX$, such that $i$th row of $\widetilde{\mX}_{\texttt{Aug}} $ is $\bx^{(i)}$, if $i\in\mathcal{E}$, otherwise is all zero vector. We first bound $T_1$ as
%     \begin{align*}
%      T_1 &= \norm{\text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{   (\bx^{(i)})^\top     \widehat{\mW}_Q   }{  \widetilde \mX_{\texttt{Aug}} {\widehat{\mW}_K}  }}\widetilde \mX_{\texttt{Aug}}  \widehat{\mW}_{V} - \text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{ (\bx^{(i)} )^\top    \widehat{\mW}_Q   }{    \mX {\widehat{\mW}_K}  }}  q\mX  \widehat{\mW}_{V}}^2 \\  
%          & \leq 2\norm{\text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{   (\bx^{(i)})^\top     \widehat{\mW}_Q   }{  \widetilde \mX_{\texttt{Aug}} {\widehat{\mW}_K}  }}\widetilde \mX_{\texttt{Aug}}  \widehat{\mW}_{V} - \text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{ (\bx^{(i)} )^\top    \widehat{\mW}_Q   }{    \widetilde \mX_{\texttt{Aug}}{\widehat{\mW}_K}  }}  q\mX  \widehat{\mW}_{V}}^2 \\  
%          & + 2\norm{\text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{   (\bx^{(i)})^\top     \widehat{\mW}_Q   }{  \widetilde \mX_{\texttt{Aug}} {\widehat{\mW}_K}  }}  q\mX   \widehat{\mW}_{V} - \text{Softmax}\pare{\frac{1}{\sqrt{d_K}}\inprod{ (\bx^{(i)} )^\top    \widehat{\mW}_Q   }{    \mX {\widehat{\mW}_K}  }}  q\mX  \widehat{\mW}_{V}}^2 \\  
%          & \leq 2\norm{ \widetilde \mX_{\texttt{Aug}}   -   q \mX  }^2 \norm{\widehat{\mW}_{V}}^2 + 2\frac{1}{\tau^2 d_K}\norm{   \inprod{   (\bx^{(i)})^\top     \widehat{\mW}_Q   }{  \widetilde \mX_{\texttt{Aug}} {\widehat{\mW}_K}  }    -    \inprod{ (\bx^{(i)} )^\top    \widehat{\mW}_Q   }{    \mX {\widehat{\mW}_K}  }   }^2 \norm{q\mX  \widehat{\mW}_{V}}^2\\
%          & \leq 2\norm{ \widetilde \mX_{\texttt{Aug}}   -  q \mX  }^2 \norm{\widehat{\mW}_{V}}^2 + 2\frac{1}{\tau^2 d_K}\norm{ \bx^{(i)}   }^2\norm{  \widetilde \mX_{\texttt{Aug}}    -     \mX    }^2 \norm{\widehat{\mW}_K}^2\norm{q\mX}^2\norm{  \widehat{\mW}_{V}}^2\\
%     \end{align*}

      
%       where we used $\frac{1}{\tau}$ Lipschitzness of softmax function. 
      
      
%       Putting pieces together yields:
%       \begin{align*}
%           &\E_{\cM} \norm{( {h}_{\texttt{Aug}} (\widetilde \mX) + \mW) -  q{h}(\mX)}^2\\
%           &\leq  \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}}  \left(2\norm{ \widetilde \mX_{\texttt{Aug}}   -  q \mX  }^2 \norm{ {\mW}_{V}}^2 + 2\frac{1}{\tau^2 d_K}\norm{ \bx^{(i)}   }^2\norm{  \widetilde \mX_{\texttt{Aug}}    -     \mX    }^2 \norm{ {\mW}_K}^2\norm{q\mX}^2\norm{{\mW}_{V}}^2 \right.\\
%           &\qquad   \qquad  \qquad \qquad\left.+2\norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2 \norm{\ind{i\in\mathcal{E}}\bx^{(i)}- q\bx^{(i)}}^2\right) \\
%           &\quad + 2\E_{\cM} \sum_{i=1}^K\ind{i\notin \mathcal{E}} \norm{\bw - q{h}^{(i)}(\mX)}^2 \\
%       \end{align*}
%       Now we derive the bound piece by piece. First, we study $ \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{ \widetilde \mX_{\texttt{Aug}}   -   q\mX  }^2$ term:
%        \begin{align*}
%           \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{ \widetilde \mX_{\texttt{Aug}}   -  q\mX  }^2& =  \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \sum_{j=1}^K\norm{ \ind{j\in \mathcal{E}}\bx^{(j)}  -   q\bx^{(j)}  }^2\\
%           &=  \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \sum_{j=1}^K \pare{\ind{j\in \mathcal{E}}\norm{ \bx^{(j)}  -   q\bx^{(j)}  }^2  + \ind{j\notin \mathcal{E}}\norm{   q\bx^{(j)}  }^2 }\\
%           &=  \E_{\cM} \sum_{(i,j)\in [K]\times[K]}  \ind{i\in \mathcal{E}} \pare{\ind{j\in \mathcal{E}}\norm{ \bx^{(j)}  -   q\bx^{(j)}  }^2  +   \ind{j\notin \mathcal{E}}\norm{   q\bx^{(j)}  }^2 }\\
%           &=    p(1-q)^2\sum_{i=1}^K \norm{\bx^{(i)}}^2 \\
%           &\quad +\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \sum_{j\in [K],j\neq i}  \pare{\ind{j\in \mathcal{E}}\norm{ \bx^{(j)}  -   q\bx^{(j)}  }^2  + \ind{j\notin \mathcal{E}}\norm{   q\bx^{(j)}  }^2 }\\
%             &=    p(1-q)^2\sum_{i=1}^K \norm{\bx^{(i)}}^2   + p (K-1)\sum_{i=1}^K\pare{p(1-q)^2\norm{ \bx^{(j)}  }^2  + (1-p)\norm{   q\bx^{(j)}  }^2 }\\
%           & =  \sum_{i=1}^K   \pare{p(1-q)^2 + p^2 (K-1)(1-q)^2 + pq^2(K-1)(1-p)} \norm{\bx^{(i)}}^2 \\
%           &=  \pare{p(1-q)^2 + p^2 (K-1)(1-q)^2 + pq^2(K-1)(1-p)} \norm{\mX}_{\mathrm{F}}^2.
%       \end{align*}
%       Then we switch to bound $ \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2 \norm{ \widetilde \mX_{\texttt{Aug}}   -  \mX  }^2 $:
%         \begin{align*}
%             \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2 \norm{ \widetilde \mX_{\texttt{Aug}}   -  \mX  }^2 =\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2 \sum_{j=1}^K \norm{ \ind{j\in\mathcal{E}}\bx^{(j)}   -  \bx^{(j)} }^2 
%         \end{align*}
%         Since $\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2  \norm{ \ind{i\in\mathcal{E}}\bx^{(j)}   -  \bx^{(j)} }^2 =0$, we have:
%        \begin{align*}
%             \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2 \norm{ \widetilde \mX_{\texttt{Aug}}   -  \mX  }^2 &=\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\bx^{(i)}}^2 \sum_{j\in[K],j\neq i} \norm{ \ind{j\in\mathcal{E}}\bx^{(j)}   -  \bx^{(j)} }^2 \\
%             &=  \sum_{i=1}^K p \norm{\bx^{(i)}}^2 \sum_{j\in[K],j\neq i}  (1-p) \norm{ \bx^{(j)} }^2\\ 
%             &\leq p(1-p) \norm{\mX}^4_{\mathrm{F}}.
%         \end{align*}

%         Now, we have to bound $\E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\ind{i\in\mathcal{E}} \bx^{(i)} - q \bx^{(i)}}^2$ as 
%         \begin{align*}
%             \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \norm{\ind{i\in\mathcal{E}} \bx^{(i)} - q \bx^{(i)}}^2 &= \E_{\cM} \sum_{i=1}^K\ind{i\in \mathcal{E}} \pare{\ind{i\in\mathcal{E}}\norm{ \bx^{(i)} - q \bx^{(i)}}^2+\ind{i\notin\mathcal{E}} \norm{ q \bx^{(i)}}^2}\\
%            & =   \sum_{i=1}^K p  (1-q)^2\norm{ \bx^{(i)}  }^2  = p(1-q)^2 \norm{\mX}_{\mathrm{F}}^2.
%         \end{align*}
%         Putting pieces together yields:
%         \begin{align*}
%           &\E_{\cM} \norm{( {h}_{\texttt{Aug}} (\widetilde \mX) + \mW) -  q{h}(\mX)}^2\\
%           &\leq   2\pare{p(1-q)^2 + p^2 (K-1)(1-q)^2 + pq^2(K-1)(1-p)} \norm{\mX}_{\mathrm{F}}^2\\
%           &+ \frac{2pq^2(1-p)}{\tau^2 d_K} \norm{\mW_K}^2 \norm{\mW_V}^2 \norm{\mX}_{\mathrm{F}}^6  +2 \norm{\mW_{\texttt{FC1}}}^2\norm{\mW_{\texttt{FC2}}}^2 p(1-q)^2 \norm{\mX}_{\mathrm{F}}^2   + 2\E_{\cM} \sum_{i=1}^K\ind{i\notin \mathcal{E}} \norm{\bw - q{h}^{(i)}(\mX)}^2 \\
%       \end{align*}
%   The last term can be bounded as:
%   \begin{align*}
%       \E_{\cM} \sum_{i=1}^K\ind{i\notin \mathcal{E}} \norm{\bw - q{h}^{(i)}(\mX)}^2 = \E_{\cM} \sum_{i=1}^K\ind{i\notin \mathcal{E}} \pare{ \norm{\bw}^2  - q\bw^\top{h}^{(i)}(\mX) +q^2\norm{{h}^{(i)}(\mX)}^2}\\
%       =(1-p) \pare{ K\norm{\bw}^2 - q\sum_{i=1}^K \bw^\top {h}^{(i)}(\mX)  + q^2 \norm{h(\mX)}^2_{\mathrm{F}} },
%   \end{align*}
%   which concludes the proof.
%    \end{proof}
% \end{lemma}

% \begin{align*}
%     T_{ij} &\geq - \frac{W^2}{K} \underbrace{\norm{\E_{\cM,\mX}\spare{(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i\bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) - q^2\hat h^\top ( \mX) \be_1\be_1^\top \hat h (  \mX) }}}_{A} \\
%      &\quad -2\frac{W^2}{K}\underbrace{\norm{\E_{\cM,\mX}\spare{(h^*_{\texttt{Aug}}  (\widetilde \mX) + \mW_{\texttt{Pad}})^\top{\bs^*_i} \bs_i^\top (\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) -   q^2(h^*(\mX))^\top\be_1\be_1^\top \hat h(\mX)} }}_{B} \\
%       &\quad - \frac{W^2}{K}\underbrace{\norm{\E_{\cM,\mX}\spare{(h^*_{\texttt{Aug}}  (\widetilde \mX) + \mW_{\texttt{Pad}})^\top{\bs^*_i} \bs^*_i^\top (  h^*_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) -   q^2(h^*(\mX))^\top\be_1\be_1^\top  h^*(\mX)}}}_{C} \\
% \end{align*} 

% For $A$, we have:
% \begin{align*}
%     A &\leq \E_{\cM,\mX}\norm{\spare{(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i\bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) - q^2\hat h^\top ( \mX) \be_1\be_1^\top \hat h (  \mX) }}\\
%     &\leq  \E_{\cM,\mX}\norm{ (\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i\pare{\bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) - q \be_1^\top \hat h (  \mX) } }\\
%     &\quad + \E_{\cM,\mX}\norm{\pare{(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i - q \hat h^\top ( \mX) \be_1}q\be_1^\top \hat h (  \mX) }\\
%     &\leq \frac{1}{2}\spare{\underbrace{\E_{\cM,\mX}\norm{ (\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i}^2}_{I}+\underbrace{\E_{\cM,\mX}\norm{\pare{\bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) - q \be_1^\top \hat h (  \mX) } }^2}_{II}}\\
%     &\quad+\frac{1}{2}\spare{\underbrace{\E_{\cM,\mX}\norm{\pare{(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}})^\top\bs_i - q \hat h^\top ( \mX) \be_1}}^2}_{III} +\underbrace{\E_{\cM,\mX}\norm{q\be_1^\top \hat h (  \mX) }^2}_{IV} }\\
% \end{align*}

% For (I), we have
% \begin{align*}
%     I \leq \norm{ \widehat\mW_V}^2  ((K-1)p^2 + pK)\norm{\mX}^2_{\mathrm{F}} + K(1-p)\norm{\bw_{\texttt{Pad}}}^2 \leq O(p^2 + p ),\\
% \end{align*}
% where we use the fact that with probability at least $$
% \begin{align*}
%     II &\leq 2 \E_{\cM,\mX}\norm{\pare{\bs_i^\top(\hat h_{\texttt{Aug}}(\widetilde \mX)+ \mW_{\texttt{Pad}}) - q \bs_i^\top \hat h (  \mX) } }^2 + 2\E_{\cM,\mX}\norm{\pare{q \bs_i^\top \hat h (  \mX) - q \be_1^\top \hat h (  \mX) } }^2\\
%     &\leq 2\pare{p(1-q)^2 + p^2 (K-1)(1-q)^2 + pq^2(K-1)(1-p)} \norm{\mX}_{\mathrm{F}}^2\\
%           &+ \frac{2pq^2(1-p)}{\tau^2 d_K} \norm{\widehat\mW_K}^2 \norm{\widehat\mW_V}^2 \norm{\mX}_{\mathrm{F}}^6  +2 \norm{\widehat\mW_{\texttt{FC1}}}^2\norm{\widehat\mW_{\texttt{FC2}}}^2 p(1-q)^2 \norm{\mX}_{\mathrm{F}}^2  \\
%           &+ 2(1-p) \pare{ K\norm{\bw}^2 - q\sum_{i=1}^K \bw^\top {\hat h}^{(i)}(\mX)  + q^2 \norm{\hat h(\mX)}^2_{\mathrm{F}} } + 4 q^2 \norm{\widehat\mW_{\texttt{FC1}}}^2\norm{\widehat\mW_{\texttt{FC2}}}^2\pare{2\norm{\widehat \mW_V}^2\norm{\mX }^2 + 2\norm{\mX}^2}\\
%           & \leq O\pare{p(1-q)^2 +   p^2 (1-q)^2 +  pq^2 (1-p) + { p(1-p)q^2}   +p(1-q)^2 + (1-p)q + (1-p)q^2 + q^2 }
% \end{align*}

% if we choose $q = p$, we have:
% \begin{align*}
%    II \leq  O\pare{p(1-p)^2 + p^2 (1-p)^2 +p^3(1-p) + (1-p)p + (1-p)p^2 + p^2 }
% \end{align*}
% \textcolor{red}{stop here --------------------------------------------------}


==> discussion.tex <==
\section{Discussion and Future Works}\label{sec: discussion}
In this paper, we proved
that both Local GD and Local SGD that are originally proposed for communication efficient network training can achieve global minima of the training loss for over-parameterized
deep ReLU networks. We make the first theoretical trial on the analysis of Local (S)GD on training Deep ReLU network, but we do not claim that our results, e.g., number of required neurons and dependency on the number of layers, are optimal in any sense. A number of future works/improvements are still exciting to explore.


\noindent\textbf{Tightening the condition on the number of neurons.}~In both Local GD and SGD bound,we require the number of neurons to have a heavy dependency on $n$, worse than the single machine case. We are aware of some recent works~\cite{noy2021convergence,nguyen2020global,nguyen2021proof} that have significantly reduced the  number of required neuron, and  we believe incorporating their results can also improve our theory.

\noindent\textbf{Extension of analysis to other federated optimization methods.} To further reduce the harm caused by multiple local updates, a line of recent studies proposed alternative methods to reduce the  local model deviation~\cite{karimireddy2019scaffold,yuan2020federated}. Establishing the  convergence of these variants on deep non-smooth networks is another valuable research direction.  
 
 
\noindent\textbf{Extension to other neural network architectures.} In this paper we only consider simple ReLU forward feed neural network, but as shown in the prior works~\cite{allen2019convergence,zou2020global}, single machine SGD can optimize more complicated neural network like CNN, ResNet or RNN as well. Hence, one natural future work is to extend our analysis on Local SGD to those neural network model.

==> end_to_end_proofs.tex <==
\section{Proof of Generalization of End-to-end Fine-tuning with Gradient Descent}\label{app:endtoend}

In this section we are going to provide detailed setup and formal result in Section~\ref{sec:nofreezing} on the generalization of end-to-end fine-tuning. Here we consider an $L$ layer neural network as encoder, followed by a fully connected layer as deconder. In downstream task, we discard decoder and add another fully connected layer on top of encoder network and jointly update them.

\textbf{Pre-training stage}
We first initialize each row $\mW_l^0$ as Gaussian distribution $\cN(0,\frac{2\mI}{m})$, for all $l\in[L+1]$. Pre-training objective is 
\begin{align*}
    &\min_{ g \in \cG,  h  \in \cH} \cL_{\widehat\cU} (g\circ h) := \frac{1}{N}\sum_{i=1}^N \norm{g\circ h(\tilde\bz_i)- \tilde \by_i}^2, 
\end{align*}



The updating rule is: for iterations $t= 0,...,T-1$:
\begin{align}
    \mW^{t+1}_l = \mW^{t}_l - \eta \nabla_{\mW_l} \cL_{\widehat{\cU}} \pare{\mW^t_{[L+1]}},\quad \quad \forall l\in[L+1]. \label{eq: GD pretrain}
\end{align}
where with slightly abuse of notation we write loss function $\cL_{\widehat{\cU}}$ is a function of model parameters.
\textbf{Fine-tuning stage}
When we finish pre-training, we will get encoder layers' weights $\mW^T_1,...,\mW^T_L$. Next in fine-tuning stage, we use these weights as initialization as well as initialize each row of $\mtheta^0$ by  $\cN(0,\frac{2\mI}{m})$, and run another $T$ iterations of gradient descent on them jointly with optimizing classification head $\boldsymbol{\Theta}$ on the following objective
\begin{align*} 
      \min_{ f \in \cF,  h  \in \cH} \cR_{\widehat\cT} (f\circ h) := \frac{1}{n} \sum_{i=1}^n \phi\pare{f\circ h(\bx_i),y_i}.
\end{align*}
where $\phi(z) = \log(1+\exp(-z))$.
The updating rule is: for iterations $t= 0,...,T-1$
\begin{align}
    \mW^{T+t+1}_l &= \mW^{T+t}_l - \gamma \nabla_{\mW_l}\cR_{\widehat{\cT}} \pare{\boldsymbol{\Theta}^t, \mW^{T+t}_{[L]}},  \quad  \quad \forall l\in[L] ,\label{eq: GD ft 1}\\
    \boldsymbol{\Theta}^{t+1} &=  \boldsymbol{\Theta}^{t} - \nabla_{ \boldsymbol{\Theta}}\cR_{\widehat{\cT}} \pare{\boldsymbol{\Theta}^t, \mW^{T+t}_{[L]}}.\label{eq: GD ft 2}
\end{align}
 At last, we use $ \boldsymbol{\Theta}^T, \mW_1^{2T},...,\mW_L^{2T}$ as our final model $\hat{f}, \hat{h}$.  


 
\paragraph{Generalization bound}
Before we present the formal generalization bound, we need to make the following two customary assumptions made in deep learning optimization theory~\cite{allen2019convergence,zou2019improved}. First, we need the data to be separable.
 \begin{assumption}
[Data Separateness]\label{assumption:separateness}
 For any two different pre-training training data points $\tilde\bz_i$ and $\tilde\bz_j$ , there exists a positive constant $c_1$ , such that $\norm{\tilde\bz_i - \tilde\bz_j} \geq c_1$. Similarly for any two different downstream training data points $ \bx_i$ and $ \bx_j$ , there exists a positive constant $c_2$ , such that $\norm{ \bx_i -  \bx_j} \geq c_2$. 
 \end{assumption}
% \textcolor{red}{should not this be assumption? we should clarify this and mention this in on what: representations, fine-tuned data}
 

\begin{assumption}\label{assumption: number of data}
    We assume number pre-training data and downstream data satisfy: $N \geq \Omega \pare{ (\frac{c_1}{c_2})^{1/2} n^{3/2} L^{2/3}}$.
\end{assumption}
This assumption is realizable since in most of machine learning scenario, we have tons of unlabeled pre-training data but very few downstream data.
\begin{theorem}[Formal version of Theorem~\ref{thm: end to end informal}] \label{thm:end to end formal} Assume Assumptions~\ref{assumption:separateness} and~\ref{assumption: number of data} to be satisfied. If we choose
\begin{align*}
    m \geq \frac{n^9 L^{16} (n^3\epsilon^{-1} +n^5)\sqrt{dN}}{c_2^4} \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }
\end{align*}
and  
\begin{align*}
        T =  O\pare{L^3\frac{n^3\epsilon^{-1}  - n^3 \pare{\sqrt{ {dN^2 } } \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }}^{-1} +n^5}{ c_2  }},
    \end{align*}
and utilizes  gradient descent in pre-training and fine-tuning stages to get $\hat{f}$ and $\hat{h}$, with learning rate $\eta = O(\frac{d}{m})$ and $\gamma = O(\frac{1}{mL^3})$, then with probability at least $0.99$, the following statement holds 
\begin{align*}
    \cE_{\cT} (\hat{f},\hat{h}) \leq  \epsilon +\frac{\sqrt{L}\poly_{L+1}\pare{1+  { {c_1^{3/2}   }{N^{-3} L^{-6}}}  +   {c_{2}^{3/2}}{ {n^{-9} L^{-8}}}}}{\sqrt{n}}. 
\end{align*}
for end-to-end optimization error of $0 < \epsilon < 1$. % \begin{align*}
%     \frac{\sqrt{L} \prod_{l=1}^{L+1} \pare{1+  {\frac{c_1^{3/2}  \log(N)}{N^3 L^6}}  +  \frac{c_{2}^{3/2}}{ {n^{9} L^8}}  }  }{\sqrt{n}} 
% \end{align*}
\end{theorem} 
The main difference on top of existing generalization analysis of GD-trained neural network is that, for fine-tuning stage, we are not training neural network from Gaussian initialization, but from weight matrices obtained from pre-training stage. Hence to apply the existing NTK fashion analysis, we have to show two things, one is the downstream loss at pre-trained weights will not blow up. (Notice that this is not trivial, since all existing bounded initial loss results~\cite{allen2019convergence,zou2019improved,zou2020gradient} are only proven on Gaussian initialization.) We find that the loss at pre-trained initialization is related to correlation between pre-training and fine-tuning data which can help us to overcome this technical challenge. The second issue we need to address is to show  that the weight matrices during fine-tuning based on gradient descent updates will not leave the small ball around Gaussian initialization. 

Before we delve into  the proof of Theorem~\ref{thm:end to end formal}, we first introduce some technical lemmas in the next subsection that will facilitate the proof of main result.
\subsection{Technical Lemmas}


\begin{lemma}\cite{zou2019improved} \label{lem:pretrain weight norm bound}
Let $\hat{\mW}$ be the neural network weight trained by GD with $\eta = O(\frac{d}{m})$ after $T$ iterations, and $\mW_l^0$ be initialization Gaussian matrix where each row of weight matrix $\mW_l^0$ is independently generated
from $\mathcal{N}(0,2\mI/m)$. If the training data are pair-wised separated, i.e., $\norm{\tilde\bz_i- \tilde\bz_j} \geq c_1, \forall i,j\in[N]$, then, the following facts hold true with probability least $1 - \Theta(\frac{1}{N})$:
    \begin{align*}
       \norm{ \hat{\mW}_l  - \mW_l^0 }_2 &\leq \norm{ \hat{\mW}_l  - \mW_l^0 }_{\mathrm{F}} \leq   O\pare{ \sqrt{\frac{d N^2\log(N)}{mc_1    }}\sqrt{ \cL_{\widehat \cU}(  \mW^0_{[L+1]}) } },\\
        {\cL_{\widehat \cU} (\mW^T_{[L+1]}) &\leq O\pare{1 - \frac{ c_1  }{ N^2}  }^T\cL_{\widehat \cU}(  \mW^0_{[L+1]})}.
 \end{align*} 
\end{lemma}

\begin{lemma}\cite{zou2020gradient} \label{lem: gradient bound}
For any $\widetilde{\mW}_l \in \cB(\mW_l^0, \omega)$ and $\widetilde\mtheta \in \cB(\boldsymbol{\Theta}^0, \omega)$ for $\omega = O(s)$, there exists constant $C$ such that
    \begin{align*}
     \norm{\nabla_{\widetilde\mtheta} \cR_{\widehat \cT}  (\widetilde\mtheta ,\widetilde\mW)  }^2 \geq   C  \frac{m s }{n^5} \pare{\sum_{i=1}^n \phi'( \hat{y}_i y_i  )}^2   ,\  \norm{\nabla_{\widetilde\mtheta} \cR_{\widehat \cT} (\widetilde\mtheta, \widetilde\mW) } \leq   - \frac{C' Lm^{1/2} }{n }  \sum_{i=1}^n \phi'( \hat{y}_i y_i  ) ;  \\
       \norm{\nabla_{\widetilde\mW_l} \cR_{\widehat \cT}  (\widetilde\mtheta ,\widetilde\mW)  }^2 \geq   C  \frac{m s }{n^5} \pare{\sum_{i=1}^n \phi'( \hat{y}_i y_i  )}^2   ,\  \norm{\nabla_{\widetilde\mW_l} \cR_{\widehat \cT} (\widetilde\mtheta, \widetilde\mW) } \leq   - \frac{C' Lm^{1/2} }{n }  \sum_{i=1}^n \phi'( \hat{y}_i y_i  ) .   
 \end{align*} 
\end{lemma}
\begin{lemma}[Output bound at Gaussian initialization]\label{lem:initial loss gaussian}
Let $h_l^0(\bx) = \sigma(\mW_l^0\cdots \sigma(\mW_1^0\bx))$ be the $l$th layer output of encoder at Gaussian initialization.
With probability at least $1-\nu$, the loss at Gaussian initialization satisfies $ \norm{h_l^0(\bx_i
)} \leq O(1+l\sqrt{\frac{\log(nL/\nu)}{m}}).$
\end{lemma}
Above lemma characterizes the boundedness of encoder output, but unfortunately, it is under Gaussian initialization. What we care more about is the boundedness of output at pre-trained initialization. Notice that it is not straightforward, since we pre-train the encoder using pre-training data $\tilde \bz_i$ but evaluate the output at downstream data $\bx_i$. Hence, we first derive the following lemma to show that after pre-training, the output of encoder will not drift far away from Gaussian initialization.

\begin{lemma}  \label{lem: output bound}
Let $h_l^t(\bx) = \sigma(\mW_l^t\cdots \sigma(\mW_1^t\bx))$ be the $l$th layer output of encoder.
If we choose $\eta  = O(\frac{d}{m})$, then the following statement holds:
    \begin{align*}
       \norm{ h^T_1(\bx_i) - h_1^0(\bx_i)}^2 \leq      O\pare{ \sqrt{\frac{dN^2 }{mc_1} }  }  \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}  + O\pare{ L\sqrt{\frac{d N^2\log(N)}{mc_1    }}  } .     
 \end{align*} 
 \begin{proof}
     For $l=1$:
     \begin{align*}
         \norm{ h^T_1(\bx_i) - h_1^0(\bx_i)}& = \norm{\sigma(\mW_1^T\bx_i) - \sigma(\mW_1^0\bx_i)} \leq \norm{\eta \sum_{t=1}^T \nabla_{\mW_1} \cL_{\widehat \cU}(\mW_{[L+1]}^t) \bx_i}\\
         &\leq \eta \sum_{t=1}^T O\pare{\sqrt{m/d} \sqrt{\cL_{\widehat\cU}(\mW^t_{[L+1]})}} \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i} \\
         & \leq \eta \sum_{t=1}^T O\pare{\sqrt{m/d} \sqrt{\pare{1-\frac{c_1}{N^2}}^t}} \max_{j\in[N]}\abs{  \tilde \bz^\top_j \bx_i}\\
           & \leq \eta   O\pare{\sqrt{\frac{N^2m}{dc_1} }  }  \max_{j\in[N]}\abs{  \tilde \bz^\top_j \bx_i},
     \end{align*}
     where the first inequality follows~\cite{allen2019convergence}, Appendix~9.1.
     
     For $l+1$:
     \begin{align*}
         \norm{ h^T_{l+1}(\bx_i) - h_{l+1}^0(\bx_i)}& = \norm{\sigma(\mW_{l+1}^T h^T_{l }(\bx_i) ) - \sigma(\mW_{l+1}^0 h_{l }^0(\bx_i))} \\ 
         & = \norm{ \mW_{l+1}^T  -  \mW_{l+1}^0 }\norm{h_{l }^T(\bx_i)}  +\norm{\mW_{l+1}^0}\norm{h_{l }^T(\bx_i) - h_{l }^0(\bx_i) }\\
           & \leq  \norm{ \mW_{l+1}^T  -  \mW_{l+1}^0 }\norm{h_{l }^0(\bx_i)} + \norm{ \mW_{l+1}^T  -  \mW_{l+1}^0 }\norm{h_{l }^T(\bx_i)-h_{l }^0(\bx_i)} \\ 
           &\quad +\norm{\mW_{l+1}^0 }\norm{h_{l }^T(\bx_i) - h_{l }^0(\bx_i) }\\ 
           & \leq  \norm{ \mW_{l+1}^T  -  \mW_{l+1}^0 }\norm{h_{l }^0(\bx_i)}  \\ 
           &\quad +\pare{\norm{\mW_{l+1}^0 }+\norm{ \mW_{l+1}^T  -  \mW_{l+1}^0 }}\norm{h_{l }^T(\bx_i) - h_{l }^0(\bx_i) }.
     \end{align*}
     Now we plug in Lemma~\ref{lem:pretrain weight norm bound}
        \begin{align*}
         \norm{ h^T_{l+1}(\bx_i) - h_{l+1}^0(\bx_i)}   
           & \leq  O\pare{ \sqrt{\frac{d N^2\log(N)}{mc_1    }}  }\norm{h_{l }^0(\bx_i)}   +    O\pare{1+ \sqrt{\frac{d N^2\log(N)}{mc_1    }} } \norm{h_{l }^T(\bx_i) - h_{l }^0(\bx_i) }\\ 
           & \leq O\pare{1+ \sqrt{\frac{d N^2\log(N)}{mc_1    }} }^{l-1} \norm{h_{1 }^T(\bx_i) - h_{1 }^0(\bx_i) }\\
           &\quad +\sum_{l'=1}^l  O\pare{1+ \sqrt{\frac{d N^2\log(N)}{mc_1    }} }^{l'}O\pare{ \sqrt{\frac{d N^2\log(N)}{mc_1    }}  }   \\ 
           & \leq O\pare{1+ \sqrt{\frac{d N^2\log(N)}{mc_1    }} }^{L}   O\pare{ \eta\sqrt{\frac{N^2m}{dc_1} }  }  \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}  + O\pare{ L\sqrt{\frac{d N^2\log(N)}{mc_1    }}  }  . 
     \end{align*}
     where in the second inequality we use the fact that $\norm{h_{l }^0(\bx_i)} \leq O(1)$.
 \end{proof}
\end{lemma}

Next we need to show that, if we use pre-trained encoder layers $\mW_1^T,...,\mW_l^T$ as the initialization for downstream task, the downstream loss will not be very large, which is captured by the following lemma:
\begin{lemma} 
[Initial loss of pre-trained encoder on downstream task]\label{lem:initial loss}
Let $\mtheta^0$ be downstream Gaussian initilization and $\mW_{[L]}^T$ be pre-trained weight matrices. Then the following statement holds with probability at least $1-\nu$:
    \begin{align*}
        \cR_{\widehat{\cT}} \pare{\mtheta^0,\mW_{[L]}^T } \leq O\pare{\sqrt{ {dN^2\log(1/\nu)} }} \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }
    \end{align*}
    \begin{proof}
        Recall that in downtream task, our neural network at initialization looks like:
        \begin{align*}
            \hat{y}_i = \bu^\top \sigma\pare{\mtheta^0\sigma(\mW_L^T\cdots\sigma(\mW_1^T\bx_i))}
        \end{align*}
        where we use $\hat{y}_i$ to denote output when input is $\bx_i$. Also recall that $\bu\in\R^m$ is chosen such that the first half coordinates are $1$ and rest are $-1$. Hence, we can compute output at initialization as:
        \begin{align*}
            \hat{y}_i = \sum_{r=1}^{m/2} \pare{\sigma( \btheta_r^\top h_L^T(\bx_i) ) -\sigma(    \btheta_{r+m/2}^\top h_L^T(\bx_i))}
        \end{align*}
        where we use $\btheta_r$ to denote $r$th row of $\mtheta^0$. 

        \begin{align*}
            \left| \norm{h_L^T(\bx_i)} - 1  \right| &\leq   \left| \norm{h_L^0(\bx_i)}  - 1  \right| +   \left| \norm{h_L^T(\bx_i)} - \norm{h_L^0(\bx_i)}  \right| \\
           & \leq O\pare{L\sqrt{\frac{\log(NL/\nu)}{m}}} + \norm{h_L^T(\bx_i)  -  h_L^0(\bx_i)} \\
            &\leq O\pare{L\sqrt{\frac{\log(NL/\nu)}{m}}} +  O\pare{ \sqrt{\frac{dN^2 }{mc_1} }  }  \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}  + O\pare{ L\sqrt{\frac{d N^2\log(N)}{mc_1    }}  }.
        \end{align*}
        where at second inequality we apply Lemma~\ref{lem:initial loss gaussian}, and at last inequality we evoke Lemma~\ref{lem: output bound}.
        We examine the range of each individual summand:
        \begin{align*}
            \norm{\sigma( \btheta_r^\top h_L^T(\bx_i) ) -\sigma(    \btheta_{r+m/2}^\top h_L^T(\bx_i))}_{\psi_2} \leq  O\pare{\sqrt{\frac{dN^2\log(1/\nu)}{m}}} \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }
        \end{align*}
        Hence by concentration we have with probability at least $1-\nu$
        \begin{align*}
            |\hat{y}_i - \E[\hat{y}_i] | &=|\hat{y}_i - 0 | \leq \sqrt{\sum_{r=1}^{m/2} \norm{\sigma( \btheta_r^\top h_L^T(\bx_i) ) -\sigma(    \btheta_{r+m/2}^\top h_L^T(\bx_i))}^2_{\psi_2}\log(1/\nu)}\\
           & \leq  O\pare{\sqrt{ {dN^2\log(1/\nu)} }} \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }.  
        \end{align*}
        Consequently,  we have 
        \begin{align*}           
        \cR_{\widehat\cT} (\mtheta^0,\mW^T_{[L]}) & = \frac{1}{n}\sum_{i=1}^n \log(1+\exp(-y_i \hat{y}_i))  \\
        & \leq  O\pare{\sqrt{ {dN^2\log(1/\nu)} }} \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }.
        \end{align*}
        % Next, we do the following decomposition:
        % \begin{align*}
        %     \hat{y}_i &\leq \sum_{r=1}^{m/2} \pare{ \btheta_r^\top h_L^0(\bx_i) -    \btheta_{r+m/2}^\top h_L^0(\bx_i)}\\
        %     &\quad + \sum_{r=1}^{m/2} \pare{ \btheta_r^\top h_L^T(\bx_i) -   \btheta_r^\top h_L^0(\bx_i)}+ \sum_{r=1}^{m/2} \pare{ \btheta_{r+m/2}^\top h_L^T(\bx_i) -   \btheta_{r+m/2}^\top h_L^0(\bx_i)}\\
        %     &\leq O(\sqrt{\log(n/\nu)})  + \sum_{r=1}^{m/2} \norm{ \btheta_r}\norm{ h_L^T(\bx_i) -   \btheta_r^\top h_L^0(\bx_i)}+ \sum_{r=1}^{m/2} \norm{ \btheta_{r+m/2}}\norm{ h_L^T(\bx_i) -   \btheta_r^\top h_L^0(\bx_i)}\\
        %      &\leq O(\sqrt{\log(n/\nu)})  + O(\sqrt{m})\norm{ h_L^T(\bx_i) -   \btheta_r^\top h_L^0(\bx_i)} \\
        %        &\leq O(\sqrt{\log(n/\nu)})  + O(\sqrt{m})\pare{ O\pare{ \eta\sqrt{\frac{N^2m}{dc_1} }  }  \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}  +O(L) \norm{h_{l }^0(\bx_i)}} \\
        % \end{align*}
    \end{proof}
\end{lemma}

\subsection{Proof of Theorem~\ref{thm:end to end formal}}
\begin{proof}
   We first show that GD will drive the downstream training loss to zero if all iterates $\mtheta^t, \mW_{[L]}^{T+t}$ are within $\cB(\mtheta^0, \omega), \cB(\mW_l^0, \omega)$ where $\omega = O(c_2^{3/2} n^{-9/2} L^{-8}   +  {c_1^{3/2}   }{N^{-3} L^{-6}} )$. By our assumption, $N\geq n^{3/2}$, so we know  
   $\omega = O(c_2^{3/2} n^{-9/2} L^{-8}   +  {c_1^{3/2}   }{N^{-3} L^{-6}} ) \leq O(c_2^{3/2} n^{-9/2} L^{-8} )$. Hence, we can apply the result from ~\cite{zou2020gradient} (proof of Theorem 4.4):
    \begin{align*}
        T\gamma \leq O\pare{\frac{ n^5}{mc_2 } }+ O\pare{\frac{n^3\pare{\cR^{-1}_{\widehat \cT} (\mtheta^t, \mW_{[L]}^{T+t}) - \cR^{-1}_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) }}{mc_2}}
    \end{align*}
    % Re-arranging terms yields:
    % \begin{align*}
    %     \cR_{\widehat \cT} (\mtheta^t, \mW_{[L]}^{T+t}) &\leq O\pare{ \frac{n^3}{mc_2 T\gamma - n^5 + n^3/\cR_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) } }  \\
    %     &\leq O\pare{ \frac{n^3}{mc_2 T\gamma - n^5 + n^3/ O\pare{\sqrt{ {dN^2\log(1/\nu)} }} \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }} }  \\
    % \end{align*}
    
    To make sure the above loss is less or equal to $\epsilon$, we need
    \begin{align*}
        T = O\pare{\frac{n^3\epsilon^{-1} - n^3 \pare{ \sqrt{ {dN^2\log(1/\nu)} } \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }}^{-1} +n^5}{mc_2 \gamma}}
    \end{align*}
iterations of GD,    where we plug the bound for initial loss (Lemma~\ref{lem:initial loss}).
    By plugging in $\gamma = O(\frac{1}{mL^3})$, we get
    \begin{align*}
        T =  O\pare{L^3\frac{n^3\epsilon^{-1} - n^3 \pare{\sqrt{ {dN^2 } } \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }}^{-1} +n^5}{ c_2  }}
    \end{align*}
    
  
    Now we inductively show that $\mW_l^{T+t} \in \cB(\mW_l^0, \omega)$  where $\omega = O(c_2^{3/2} n^{-9/2} L^{-8}   +  {c_1^{3/2}   }{N^{-3} L^{-6}} )$ 
    For base case $t=0$:
    according to~\cite{zou2019improved} we know the pre-trained weights satisfy
      \begin{align*} 
         \norm{\mW_l^T - \mW_l^0} \leq O\pare{  {c_1^{3/2}   }{N^{-3} L^{-6}} }
    \end{align*}
   Then we assume the condition holds for any $k\leq t$. According to~\cite{zou2020gradient}, we know
    \begin{align*}
        \norm{\mW_l^{T+t} - \mW_l^T} &\leq\sqrt{2T\gamma \cR_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) } \\
        &\leq O\pare{ \sqrt{\frac{n^3\epsilon^{-1}   +n^5 }{mc_2  }\cR_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) }}
    \end{align*}
    Also by~\cite{zou2020gradient}, we know
    \begin{align*}
       \gamma \norm{\nabla  \cR_{\widehat \cT} (\mtheta^t, \mW_{[L]}^{T+t})} \leq O(\frac{1}{L^2 \sqrt{m}})
    \end{align*}
    hence we can conclude  that 
    \begin{align*}
        \norm{\mW_l^{T+t+1} - \mW_l^T} &\leq \norm{\mW_l^{T+t} - \mW_l^T} + \gamma \norm{\nabla  \cR_{\widehat \cT} (\mtheta^t, \mW_{[L]}^{T+t})} \\
        &\leq O\pare{ \sqrt{\frac{n^3\epsilon^{-1} +n^5 }{mc_2  }\cR_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) }} + O\pare{\frac{1}{L^2 \sqrt{m}}}.
    \end{align*}
    We plug in the bound for $\cR_{\widehat \cT} (\mtheta^0, \mW_{[L]}^T) $ from Lemma~\ref{lem:initial loss} to get
    \begin{align*}
        \norm{\mW_l^{T+t+1} - \mW_l^T}   &\leq O\pare{ \sqrt{\frac{n^3\epsilon^{-1} +n^5 }{mc_2  } \sqrt{ {dN^2 } }  \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }}} + O(\frac{1}{L^2 \sqrt{m}})
    \end{align*}
    To make sure all parameters  stay in the $\cB(\mW_l^0,\omega)$, we need to have
    $$m \geq \frac{n^9 L^{16} (n^3\epsilon^{-1} +n^5)\sqrt{dN}}{c_2^4} \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }, $$
    Recalling that  
    \begin{align*} 
         \norm{\mW_l^T - \mW_l^0} \leq O\pare{  {c_1^{3/2}   }{N^{-3} L^{-6}} },
    \end{align*}
    and putting pieces together will complete the proof.
\end{proof}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> nofreezing.tex <==
\section{On the Generalization of End-to-end Fine-tuning with Gradient Descent}\label{sec:nofreezing}
% \begin{lemma}
% \begin{align*}
%     \cR_{\cD}(\widehat{f} \circ \widehat{h})-\min_{f\in\cF,h\in\cH}\cR_{\cD}(f \circ h)  &\leq  \cR_{\widehat\cD}(\widehat{f} \circ \widehat{h})   + \frak{R}_{\widehat \cD}\pare{\phi\circ \cF(f_0,\widehat{h}_{\widehat \cU},\cA(\widehat \cD)) \circ \cH(f_0,\widehat{h}_{\widehat \cU},\cA(\widehat \cD))} \\
%     &\quad + \sqrt{\frac{\log(1/\nu)}{n}}
% \end{align*}
% where $\cF(f_0,\widehat{h}_{\widehat \cU},\cA(\widehat \cD))$ is the class of all encoders that can be found by algorithm $\cA$ on training set $\widehat \cD$, with the initialization encoder and decoder to be $f_0, \widehat{h}_{\widehat \cU}$, and so is $\cH(f_0,\widehat{h}_{\widehat \cU},\cA(\widehat \cD))$.
% \end{lemma}
So far we only considered linear fine-tuning, where we only update linear head and do not update encoder during fine-tuning. In this section, we study another widely used fine-tuning method, full model fine-tuning with nonlinear head, where we jointly update nonlinear task specific head and encoder in fine-tuning stage. We instantiate our theory in the following scenario, where we consider  regression as pre-training task, and a binary classification problem as fine-tuning task.  We consider an $L$-layer neural network as encoder, followed by one fully connected layer as decoder. In finetuning stage, we also consider a fully connected layer as task specific head:
\begin{align*}
 \text{\sffamily{encoder:}} \quad    h(\bx) = \sigma\pare{\mW_L\cdots \sigma(\mW_1\bx)}  , \\
  \text{\sffamily{decoder:}} \quad    g(h(\bx)) = \mV \sigma(\mW_{L+1} h(\bx)),
\end{align*}
where $\mW_1 \in \R^{m\times d}$, $\mW_2,\ldots,\mW_{L+1} \in \R^{m\times m}$, and $\mV  \in \R^{d\times m}$.
We use gradient descent to optimize pre-training and downstream tasks. First, in pre-training stage, we run $T$ steps gradient descent to optimize $
  \min_{g \in \cG, h \in \cH} \cL_{\widehat \cU} :=   \sum_{i=1}^N \norm{g(h(\tilde\bz_i)) - \bz_i }^2$ to get $\tilde{g}, \tilde{h}$.  Then, we drop the decoder layers, and use the rest layers as an encoder. A fully connected layer is added on top of encoder in fine-tuning stage, i.e., $f(h(\bx)) = \mU \sigma(\boldsymbol{\Theta}h(\bx))$,
and using $\tilde{h}$ as initialization of encoder layers, then we run another $T$ steps of gradient descent to optimize all layers on the downstream binary classification task: $
   \min_{f\in\cF, h\in\cH} \cR_{\widehat\cT}(f\circ  {h})=   \frac{1}{n}\sum_{i=1}^n \phi(f({h}(\bx_i)),y_i). $


\begin{theorem} \label{thm:end to end formal} Assume Assumptions~\ref{assumption:separateness} and~\ref{assumption: number of data} to be satisfied. If we choose
\begin{align*}
    m &\geq \frac{n^9 L^{16} (n^3\epsilon^{-1} +n^5)\sqrt{dN}}{c_2^4}\\
    &\times \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} },
\end{align*}
and  
\begin{align*}
        T &=  O\left(\frac{L^3}{c_2}\left(n^3\epsilon^{-1} +n^5 \right)\right) \\ 
       -&\frac{n^3L^3}{c_2} O\left( \pare{\sqrt{ {dN^2 } } \cdot \max\cbr{ \max_{j\in[N],i\in[n]}\abs{  \tilde \bz^\top_j \bx_i}, L\sqrt{\log(N)} }}^{-1}  \right) ,
    \end{align*}
and utilizes  gradient descent in pre-training and fine-tuning stages to get $\hat{f}$ and $\hat{h}$, with learning rate $\eta = O(\frac{d}{m})$ and $\gamma = O(\frac{1}{mL^3})$, then with probability at least $0.99$, the following statement holds 
\begin{align*}
    \cE_{\cT} (\hat{f},\hat{h}) \leq  \epsilon +\frac{\sqrt{L}\poly_{L+1}\pare{1+  { {c_1^{3/2}   }{N^{-3} L^{-6}}}  +   {c_{2}^{3/2}}{ {n^{-9} L^{-8}}}}}{\sqrt{n}}. 
\end{align*}
for end-to-end optimization error of $0 < \epsilon < 1$. % \begin{align*}
%     \frac{\sqrt{L} \prod_{l=1}^{L+1} \pare{1+  {\frac{c_1^{3/2}  \log(N)}{N^3 L^6}}  +  \frac{c_{2}^{3/2}}{ {n^{9} L^8}}  }  }{\sqrt{n}} 
% \end{align*}
\end{theorem} 

% \begin{theorem}[Informal]\label{thm: end to end informal} Assume $m$ and $T$ is properly large. If one uses gradient descent in pre-training and fine-tuning stages to get $\hat{f}$ and $\hat{h}$, then with probability at least $0.99$, the following statement holds 
% \begin{align*}
%     \cE_{\cT} (\hat{f},\hat{h}) \leq  \epsilon +\frac{\sqrt{L}\poly_{L+1}\pare{1+  { {c_1^{3/2}   }{N^{-3} L^{-6}}}  +   {c_{2}^{3/2}}{ {n^{-9} L^{-8}}}}}{\sqrt{n}}. 
% \end{align*}

% % \begin{align*}
% %     \frac{\sqrt{L} \prod_{l=1}^{L+1} \pare{1+  {\frac{c_1^{3/2}  \log(N)}{N^3 L^6}}  +  \frac{c_{2}^{3/2}}{ {n^{9} L^8}}  }  }{\sqrt{n}} 
% % \end{align*}
% \end{theorem} 

We defer the formal theorem and all proofs in this subsection to Appendix~\ref{app:endtoend}.
\textcolor{red}{Intuitively, if in pretraining stage, we got the model that can have smaller downstream risk, then in finetuning stage, we just need few steps of GD and hence the model will not travel too far. Further, since the downstream generalization only depends on the distance that model traveled away from pretrained model, it yields better generalization.}


The main difference on top of existing generalization analysis of GD-trained neural network is, for fine-tuning stage, we are not training neural network from Gaussian initialization, but from weight matrices obtained from pre-training. Hence to apply the existing NTK fashion analysis, we have to inductively show that, the weight matrices during fine-tuning gradient descent will not leave the small ball around Gaussian initialization. Finally, the generalization bound is contributed from two parts, the distance that parameter traveled away from initialization in pre-training and that in fine-tuning.
